Dense RepPoints: Representing Visual Objects with Dense Point Sets

We present a new object representation, called Dense RepPoints, that utilizes a large set of points to describe an object at multiple levels, including both box level and pixel level. Techniques are proposed to efficiently process these dense points, maintaining near-constant complexity with increasing point numbers. Dense RepPoints is shown to represent and learn object segments well, with the use of a novel distance transform sampling method combined with set-to-set supervision. The distance transform sampling combines the strengths of contour and grid representations, leading to performance that surpasses counterparts based on contours or grids. Code is available at \url{https://github.com/justimyhxu/Dense-RepPoints}.

==> fig/figure_head.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.48\textwidth]{fig/head.pdf}
\caption{
Illustration of the head design. The attribute head is optional.}
\label{fig::head}
\end{center}
\vspace{-25pt}
\end{figure}


==> tex/application.tex <==
\subsection{Multi-Granular Representation}
\label{sec::multitask}

{\em Dense RepPoints} can also be employed to simultaneously represent multi-granular object structures, e.g. the coarse object bounding box and the more fine-grained object segment. This can be achieved by using both bounding box and segment annotation to jointly supervise the learning of {\em Dense RepPoints}. In this way, different 2D visual representations including bounding boxes, contours, and masks are unified by this dense point set representation.

Unlike Mask R-CNN \cite{Mask-rcnn} where the mask and bounding box are processed using independent branches, {\em Dense RepPoints} provides a unified representation for different granularities of object geometry. Experimental results also show that the object detection task can benefit greatly from object segments as a fine-grained supervision source even on a strong baseline, with a $+1.6$ AP improvement through this multi-granular representation (see Table~\ref{tab::multitask-points}).

\subsection{RPSeg: An Box-Free Instance Segmentation Framework}
\label{sec::framework}
\input{fig/figure_head.tex}
We design a box-free \textbf{RepPoints Segmenter (RPSeg)} for the task of instance segmentation that utilizes \emph{Dense RepPoints} as the intermediate representation throughout the pipeline. Similar to \cite{RepPoints}, we use a center point based initial object representation and utilize \emph{Dense RepPoints} as the intermediate feature sampling locations. The overall architecture is illustrated in Figure~\ref{fig::pipeline}, using an FPN backbone like in~\cite{RetinaNet, RepPoints}, where feature pyramid levels from 3 (downsampling ratio of 8) to 7 (downsampling ratio of 128) are employed. The head architecture is illustrated in Figure~\ref{fig::head}.

In addition to the class head and localization head, we introduce an optional attribute head to predict the attribute of each point. The localization subnet first computes offsets $\mathbf o_1$ for the \emph{Dense RepPoints}, then the refinement and attribute predictions are obtained by bilinear sampling on the predicted refine fields $\mathbf o_2$ and attribute maps $\mathbf a_1$ with sampling locations based on $\mathbf o_1$. For the classification branch, we use group pooling to sample the features of \emph{Dense RepPoints} with sampling locations based on $\mathbf o_1$, then fully-connected layers are used to predict the classification results. From its anchor-free design and efficient implementation in Section~\ref{sec::efficient}, our approach is fast and even more efficient than the one-stage RetinaNet \cite{RetinaNet}(215.7 vs 234.5 GFLOPS) and has a finer object representation (225 points). We use the same label assignment approach as in \cite{RepPoints}. For the additional attribute branch, we use per-point binary cross entropy for the foreground / background attribute prediction.
